Model-based functional mixture discriminant analysis with hidden process regression for curve classification

In this paper, we study the modeling and the classification of functional data presenting regime changes over time. We propose a new model-based functional mixture discriminant analysis approach based on a specific hidden process regression model that governs the regime changes over time. Our approach is particularly adapted to handle the problem of complex-shaped classes of curves, where each class is potentially composed of several sub-classes, and to deal with the regime changes within each homogeneous sub-class. The proposed model explicitly integrates the heterogeneity of each class of curves via a mixture model formulation, and the regime changes within each sub-class through a hidden logistic process. Each class of complex-shaped curves is modeled by a finite number of homogeneous clusters, each of them being decomposed into several regimes. The model parameters of each class are learned by maximizing the observed-data log-likelihood by using a dedicated expectation-maximization (EM) algorithm. Comparisons are performed with alternative curve classification approaches, including functional linear discriminant analysis and functional mixture discriminant analysis with polynomial regression mixtures and spline regression mixtures. Results obtained on simulated data and real data show that the proposed approach outperforms the alternative approaches in terms of discrimination, and significantly improves the curves approximation.

==> nettoyage <==
#!/bin/bash

function nettoie() {
  while [ -n "$1" ] ; do
    nom=$1
    rm $nom/*.toc 2>/dev/null
    rm $nom/*.mtc* 2>/dev/null
    rm $nom/*.dvi 2>/dev/null
    rm $nom/*.dvi 2>/dev/null
    rm $nom/*.out 2>/dev/null
    rm $nom/*.lof 2>/dev/null
    rm $nom/*.lot 2>/dev/null
    rm $nom/*.aux 2>/dev/null
    rm $nom/*.idx 2>/dev/null
    rm $nom/*.ilg 2>/dev/null
    rm $nom/*.ind 2>/dev/null
    rm $nom/*.log 2>/dev/null
    rm $nom/*.*# 2>/dev/null
    rm $nom/*.tex~ 2>/dev/null
    rm $nom/*.bbl 2>/dev/null
    rm $nom/*.brf 2>/dev/null
    rm $nom/*.bmt 2>/dev/null
    rm $nom/*.blg 2>/dev/null    
    rm $nom/*.snm 2>/dev/null
    rm $nom/*.nav 2>/dev/null
    rm $nom/*~ 2>/dev/null
    rm $nom/.*~ 2>/dev/null
    rm core 2>/dev/null
    echo -e '\E[34m' "Rep $nom :" '\E[0m' `ls $nom`
    shift
  done
}

nom=`pwd`
nettoie $nom

for i in `ls` ; do
	if [ -d "$i" ] ; then nettoie $i ; fi
done


